Sparse-to-Dense: Depth Prediction from Sparse Depth Samples and a Single Image

We consider the problem of dense depth prediction from a sparse set of depth measurements and a single RGB image. Since depth estimation from monocular images alone is inherently ambiguous and unreliable, to attain a higher level of robustness and accuracy, we introduce additional sparse depth samples, which are either acquired with a low-resolution depth sensor or computed via visual Simultaneous Localization and Mapping (SLAM) algorithms. We propose the use of a single deep regression network to learn directly from the RGB-D raw data, and explore the impact of number of depth samples on prediction accuracy. Our experiments show that, compared to using only RGB images, the addition of 100 spatially random depth samples reduces the prediction root-mean-square error by 50% on the NYU-Depth-v2 indoor dataset. It also boosts the percentage of reliable prediction from 59% to 92% on the KITTI dataset. We demonstrate two applications of the proposed algorithm: a plug-in module in SLAM to convert sparse maps to dense maps, and super-resolution for LiDARs. Software and video demonstration are publicly available.

==> discussion.tex <==
\section{Discussion?}

\subsection{Single CNN vs. Two-stream Network}

% In this section, we describe our common model for dense depth image prediction from different three modalities of input data, including a single RGB image, a single sparse depth image, and the combination of the two. We first present the employed architecture and then compare the performance of different components.

Most of the current cross-modality CNN architectures adopt a two-phase approach for dealing with RGBD-type data: first process raw input data of different modality separately, and then merge the them using one or multiply fully connected layers or convolution layers. While this approach proves to be successful in various object recognition tasks (see~\cite{schwarz2015rgb,gupta2014learning} and the reference therein), it gives away the opportunity to learn the low-level features that depend on both RGB and depth images, and thus essentially discards information hidden in the pixel-wise correlation between distance and color. 

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/two-stream} 
\caption{single CNN vs. two-stream network}
\label{fig:two-stream}
\end{figure}

In this work, we use one CNN architecture to solve the depth image prediction problem and demonstrate that it outperforms two-step approach on this particular task. Our hypothesis, to be borne out in experiments, is that there is enough common structure between the raw depth image and RGB images such that a network can learn a suitable representation for RGBD-type input.

We use this CNN architecture to compare between single-pipeline CNN architecture versus two-branch network and analyze 

\subsection{First Convolution Layer}

We also compare the very first convolution layer in the network and explore different possibilities. The original residual network uses a convolution. We compare the performance of using a convolution against two other choices. The first one is a depthwise separable convolution, which consists of a spatial convolution performed independently on each input channel, followed by a pointwise convolution across different channels with a windows size of 1. A second choice is channel dropout. Similar to the regular dropout commonly used for network regularization, in channel dropout each input channel is kept with some probability $p$ or set to 0 with probability $1-p$. 

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth,height=0.66\linewidth]{figures/dummy.jpg} 
\caption{feature maps}
\label{fig:features}
\end{figure}
